Manticore: Hardware-Accelerated RTL Simulation with Static Bulk-Synchronous Parallelism

The demise of Moore's Law and Dennard Scaling has revived interest in specialized computer architectures and accelerators. Verification and testing of this hardware depend heavily upon cycle-accurate simulation of register-transfer-level (RTL) designs. The fastest software RTL simulators can simulate designs at 1--1000 kHz, i.e., more than three orders of magnitude slower than hardware. Improved simulators can increase designers' productivity by speeding design iterations and permitting more exhaustive exploration. One possibility is to exploit low-level parallelism, as RTL expresses considerable fine-grain concurrency. Unfortunately, state-of-the-art RTL simulators often perform best on a single core since modern processors cannot effectively exploit fine-grain parallelism. This work presents Manticore: a parallel computer designed to accelerate RTL simulation. Manticore uses a static bulk-synchronous parallel (BSP) execution model to eliminate fine-grain synchronization overhead. It relies entirely on a compiler to schedule resources and communication, which is feasible since RTL code contains few divergent execution paths. With static scheduling, communication and synchronization no longer incur runtime overhead, making fine-grain parallelism practical. Moreover, static scheduling dramatically simplifies processor implementation, significantly increasing the number of cores that fit on a chip. Our 225-core FPGA implementation running at 475 MHz outperforms a state-of-the-art RTL simulator running on desktop and server computers in 8 out of 9 benchmarks.

==> sections/rate_model.tex <==
\begin{figure*}
    \centering
    \subfloat{\includegraphics[width=0.25\textwidth]{figures/barrier_new_rate_i7.pdf}}
    \subfloat{\includegraphics[width=0.75\textwidth]{figures/barrier_rate_epyc.pdf}}\\
    \vspace{-14pt}
    \subfloat{
      \resizebox{.85\textwidth}{!}{%
        \begin{tabular}{ l l cccccccccccc  }
          \toprule
          \multicolumn{2}{l}{\bf Instructions }     & 1.7K          & 3.5K & 6.9K & 13.8K & 27.6K & 55.3K & 110.6K & 221.2K & 442.4K & 884.7K & 1.8M & 3.5M        \\
          \midrule
          \multirow{2}{*}{\rotatebox{90}{\bf epyc}} & {\bf first }  & 1.0  & 1.3  & 1.5   & 2.2   & 2.8   & 3.9    & 5.1    & 7.6    & 10.7   & 14.2 & 18.2 & 21.7 \\
                                                    & {\bf second } & 1.1  & 1.6  & 2.1   & 2.8   & 4.0   & 5.2    & 7.9    & 11.5   & 15.9   & 21.4 & 25.6 & 28.4 \\
          \midrule
          \multirow{2}{*}{\rotatebox{90}{\bf i7}}   & {\bf first }  & 1.0  & 1.0  & 1.2   & 1.7   & 2.7   & 3.7    & 4.9    & 5.8    & 6.3    & 5.8  & 6.7  & 6.9  \\
                                                    & {\bf second } & 1.0  & 1.0  & 1.3   & 1.8   & 2.8   & 4.2    & 5.3    & 6.0    & 6.5    & 6.6  & 6.6  & 14.5 \\
          \bottomrule
        \end{tabular}
      }
    }\label{tab:fake_speedup}
    \caption{Measured parallel simulation rate on a desktop processor (left) and server processor (right). %
      Dashed lines model only synchronization cost. Solid lines also include i-cache pressure. %
      Each curve is labeled by the number of instructions executed per simulation step. %
      The table shows the speedup in each model.
    }
    \label{fig:fake_rate}
    % \end{subfigure}
  \end{figure*}
